Indiscernibles and Flatness in Monadically Stable and Monadically NIP Classes

Monadically stable and monadically NIP classes of structures were initially studied in the context of model theory and defined in logical terms. They have recently attracted attention in the area of structural graph theory, as they generalize notions such as nowhere denseness, bounded cliquewidth, and bounded twinwidth. Our main result is the - to the best of our knowledge first - purely combinatorial characterization of monadically stable classes of graphs, in terms of a property dubbed flip-flatness. A class $\mathcal{C}$ of graphs is flip-flat if for every fixed radius $r$, every sufficiently large set of vertices of a graph $G \in \mathcal{C}$ contains a large subset of vertices with mutual distance larger than $r$, where the distance is measured in some graph $G'$ that can be obtained from $G$ by performing a bounded number of flips that swap edges and non-edges within a subset of vertices. Flip-flatness generalizes the notion of uniform quasi-wideness, which characterizes nowhere dense classes and had a key impact on the combinatorial and algorithmic treatment of nowhere dense classes. To obtain this result, we develop tools that also apply to the more general monadically NIP classes, based on the notion of indiscernible sequences from model theory. We show that in monadically stable and monadically NIP classes indiscernible sequences impose a strong combinatorial structure on their definable neighborhoods. All our proofs are constructive and yield efficient algorithms.

==> chapters/extra-prelims.tex <==
\section{Additional Preliminaries}\label{sec:extra-prelims}

\paragraph*{Indiscernible sequences.}
%Let $\struc A$ be a $\Sigma$-structure and $\phi(\bar x_1,\ldots, \bar x_m)$ a formula.
%Recall that a sequence $(\bar a_i)_{1\leq i\leq n}$ of tuples from a structure $\struc A$ (where all $\bar x_i$ and $\bar a_j$ have the same length)
%is a \mbox{\emph{$\phi$-indis\-cernible sequence}} of
%length $n$, if for every two sequences of indices
%  $i_1 < \dots < i_m$ and
%  $j_1 < \dots < j_m$ from $[n]$ we have
%  \[
%  \struc A \models
%  \phi(\bar a_{i_1}, \ldots, \bar a_{i_m})
%  \quad \Longleftrightarrow \quad
%  \struc A \models \phi(\bar a_{j_1}, \ldots, \bar a_{j_m}).
%  \]
%For a set of formulas $\Delta$ we call a sequence
%\emph{$\Delta$-indiscernible} if it is $\phi$-indiscernible for
%all $\phi\in \Delta$.
For any sequence $I=(\bar a_i)_{1\leq i\leq n}$ in a structure \(\struc A\) we define the 
\emph{Ehrenfeucht-Mostowski type (EM-type)} of~$I$ as the
set of all formulas $\phi$ such that $\struc A\models \phi(\bar a_{i_1}, \ldots, \bar a_{i_m})$
for all $i_1<\ldots<i_m$. A sequence $I$ is $\Delta$-indiscernible if
and only if for all formulas $\phi\in \Delta$ either $\phi$ or $\neg\phi$ belongs to 
$\mathrm{EM}(I)$. 
Note that a subsequence $J$ of a $\phi$-indiscernible sequence $I$
is again a $\phi$-indiscernible sequence and that the
$\mathrm{EM}$-type of any subsequence $J$ of a sequence $I$ is a \emph{superset} of the $\mathrm{EM}$-type of $I$.

%For finite $\Delta$, by (iteratively applying) Ramsey's theorem we can extract
%a $\Delta$-indiscernible sequence from any sequence. In general
%structures however, in order to extract a large $\Delta$-indiscernible
%sequence we must initially start with an enormously large sequence.  To the best of our knowledge the following theorem goes back to Ehrenfeucht and Mostowski~\cite{ehrenfeucht1956models}.
%
%\begin{theorem}\label{thm:indiscernible_ramsey}
%    Let $\Delta$ be a finite set of formulas.
%    There exists a function $f$ such that every sequence of elements of length at least $f(m)$ (in a structure with a signature matching $\Delta$)
%    contains a $\Delta$-indiscernible subsequence of length $m$.
%\end{theorem}

In stable classes we can efficiently find polynomially large indiscernible sequences of elements (see also \cite[Theorem 3.5]{regularity_lemmas}). 
The theorem is stated for graphs, but it easily extends to general structures. 

\begin{theorem}[{\cite[Theorem 2.8]{kreutzer2018polynomial}}]\label{thm:extract_indiscernibles}
  Let $\CC$ be a stable class of graphs and let $\Delta$ be a finite
  set of formulas.  There is a polynomial $p(x)$ such that
  for all $G\in \CC$, every positive integer $m$ and every sequence
  $J$ of vertices of $G$ of length $\ell=p(m)$, there
  exists a subsequence $I$ of length~$m$ which is
  $\Delta$-indiscernible.

  Furthermore, there is an algorithm that given an $n$-vertex graph $G\in \CC$
  and a sequence $(v_i)_{1\leq i\leq \ell}$, computes a
  $\Delta$-indiscernible subsequence of length at
  least $m$. The running time of the algorithm is in
  $O(|\Delta| \cdot k \cdot \ell^{k+1} \cdot n^{q}\cdot a(n)\cdot \lambda(\Delta))$, where $k$
  is the maximal number of free variables, $q$ is the maximal quantifier-rank of
  a formula of $\Delta$, $a(n)$ is the time required to test adjacency between two vertices and
  $\lambda(\Delta)$ is the length of a longest formula in $\Delta$.    
\end{theorem}

By starting with a sequence $(v_i)_{1\leq i\leq \ell'}$ of length $\ell' = p(m)^{k^2+k}$, we know that the number of vertices~$n$ in the host graph is at least $\ell'$.
We may then truncate the sequence to length $\ell=p(m)$ and execute the algorithm of \Cref{thm:extract_indiscernibles}.
The factor $\ell^{k+1} = \ell'^{1/k}$ in the run time can therefore be bounded by $n^{1/k}$,
while still guaranteeing that the starting length $\ell' = p(m)^{k^2+k}$ is only polynomial in $m$.
Looking at the proof in \cite{kreutzer2018polynomial}, we see that
the time needed to evaluate $G \models \phi(\bar v)$ for formulas $\phi \in \Delta$ and tuples $\bar v$
is bounded by $\Oof(n^{q}\cdot a(n)\cdot \lambda(\Delta))$.
Over the course of this paper, we will construct indiscernibles with respect to formulas
that can be evaluated much faster.
To capture this, we only assume a generic bound $f_{\CC\Delta}(n)$ on the evaluation time for formulas in $\Delta$ on $n$-vertex graphs from~$\CC$.
Applying these two modifications to \Cref{thm:extract_indiscernibles}, we immediately get the following statement.

\begin{theorem}\label{thm:poly_seqs}
  Let $\CC$ be a stable class of graphs and let $\Delta$ be a finite set of formulas.
  Assume that we can evaluate, given $\phi \in \Delta$, an $n$-vertex graph 
  $G \in \CC$  and a tuple~$\bar v$ in $G$, whether $G \models \phi(\bar v)$ in time  
  $f_{\CC\Delta}(n)$.

  Then there is an integer $t$ and an algorithm that 
  finds in any sequence of at least $m^t$ vertices in an $n$-vertex graph $G \in\CC$ 
  a $\Delta$-indiscernible subsequence of length $m$.
  The running time of the algorithm is 
  $\Oof(|\Delta| \cdot k \cdot n^{1/k} \cdot f_{\CC\Delta}(n))$, where $k$
  is the maximal number of free variables of formulas in $\Delta$.
\end{theorem}


==> chapters/full-prelims.tex <==
\section{Preliminaries}\label{sec:prelims}

We use standard notation from graph theory and model theory
and refer to~\cite{Diestel} and~\cite{Hodges} for extensive background. 
We write $[m]$ for the set of integers $\{1,\ldots,m\}$. 
For a function $f : \NN \rightarrow \NN$ we write~$f^k(n)$ for the $k$ times iterated application of the function $f$ to the input~$n$.

\paragraph*{Relational structures and graphs.}
A \emph{(relational) signature} $\Sigma$ is a set of relation symbols, each 
with an associated non-negative integer, called its \emph{arity}.
A \emph{$\Sigma$-structure} $\struc A$ consists of a \emph{universe}, 
which is a non-empty, possibly infinite set, and \emph{interpretations} of the symbols from the
signature: each $k$-ary relation symbol is interpreted as
a $k$-ary relation over the universe. 
By a slight abuse of notation, we do not differentiate between structures and their universes and between relation symbols and their interpretations. 
By $\CC$ we denote classes of structures over a fixed signature. Unless indicated otherwise,
$\CC$ may contain finite and infinite structures.


A \emph{monadic extension} $\Sigma^+$ of a signature $\Sigma$
is any extension of $\Sigma$ by unary predicates. A unary predicate will
also be called a \emph{color}. 
A \emph{monadic expansion} or \emph{coloring} of a \mbox{$\Sigma$-structure~$\struc A$} is a $\Sigma^+$-structure~$\struc A^+$, where $\Sigma^+$
is a monadic extension of $\Sigma$, such 
that $\struc A$ is the \emph{$\Sigma$-reduct} of $\struc A^+$, that is, 
the $\Sigma$-structure obtained from $\struc A^+$ by
removing all relations with symbols in~$\Sigma^+\setminus \Sigma$.
When $\Cc$ is a class of $\Sigma$-structures and $\Sigma^+$ is a 
monadic extension of $\Sigma$, we 
write~$\Cc[\Sigma^+]$ for the class
of all possible $\Sigma^+$-expansions of structures from $\Cc$. 

A \emph{graph} is a finite structure over the signature consisting of a binary
relation symbol~$E$, interpreted as the symmetric and irreflexive edge relation.

\paragraph*{First-order logic.}
First-order logic over a signature $\Sigma$ is defined in 
the usual way.
Unless mentioned otherwise, all formulas are first-order formulas.
We usually write $\bar x$ for tuples $(x_1,\ldots, x_k)$
of variables, $\bar a$ for tuples $(a_1,\ldots, a_\ell)$ of elements and leave it to the context to determine the length of the 
tuple. We often work with \emph{partitioned formulas}, that is, formulas 
$\phi(\bar x_1, \ldots, \bar x_q)$ with a separation of the free variables. The intended partition is indicated with a comma between the tuples~of variables.

 We say that
two tuples $\bar a, \bar b$ of elements are \emph{$\phi$-connected}
in a structure $\struc A$ if $\struc A\models\phi(\bar a, \bar b)$. We call
the set $N_\phi^{\struc A}(\bar a)=\{\bar b \in \struc A^{|\bar y|}~:~\struc A\models\phi(\bar a, \bar b)\}$ the \emph{$\phi$-neighborhood} of $\bar a$. 
We simply write~$N_\phi(\bar a)$ when $\struc A$ is clear from the context. 
We remark that the $\phi$-neighborhood of $\bar a$ in model theory 
can be identified with the \emph{$\phi$-type of $\bar a$
with parameters from $\struc A$},
which is defined as 
$\{\phi(\bar a, \bar b)~:~\struc A\models\phi(\bar a,\bar b), \bar b \in \struc A^{|\bar y|}\}\cup\{\neg\phi(\bar a,\bar b)~:~\struc A\not\models\phi(\bar a,\bar b), \bar b \in \struc A^{|\bar y|}\}$. 

Let $\Phi(\bar x)$ be a finite set of formulas with free variables $\bar x$.
A \emph{$\Phi$-type}\footnote{related to, but different from the notion of a $\phi$-type with parameters from $\struc A$ mentioned in the previous paragraph} is 
a conjunction $\tau(\bar x)$ of formulas in $\Phi$
or their negations, such that every formula in $\Phi$
occurs in $\tau$ either positively or negatively.
More precisely, $\tau(\bar x)$ is a formula of the following form, for some subset $A\subseteq\Phi$:
\[\bigwedge_{\phi \in A} \phi(\bar x)\wedge  \bigwedge_{\phi \in \Phi\setminus A} \hspace{-2mm}\neg\phi(\bar x).
\]
Note that for every  $|\bar x|$-tuple $\bar a$ of elements of $\struc A$,
there is exactly one $\Phi$-type $\tau(\bar x)$ such that $\struc A\models \tau(\bar a)$.


\paragraph*{Stability and NIP.}
We refer to the textbooks \cite{baldwin2017fundamentals,pillay2008introduction,shelah1990classification, tent2012course}
for extensive background on classical stability theory. 
The most important notion in stability theory is that of \emph{stability}, 
defined as follows. 

A formula $\phi(\bar x,\bar y)$ has the \emph{$k$-order property}
on a class $\Cc$ of structures if there are $\struc A\in \Cc$ and 
two sequences $(\bar{a}_i)_{1\leq i\leq k}$, $(\bar{b}_i)_{1\leq i\leq k}$ 
of tuples of elements of $\struc A$, such that
for all $i,j\in[k]$
  \[\struc A \models \phi(\bar{a}_i,\bar{b}_j) \quad \Longleftrightarrow\quad  i \leq j.\]
  
The formula $\phi$ is said to have the \emph{order property} on $\Cc$ 
if it has the $k$-order property for all $k\in \mathbb{N}$.
The class $\Cc$
is called \emph{stable} if no first-order formula has the order-property on~$\Cc$. 
A class $\Cc$ of $\Sigma$-structures is \emph{monadically stable}
if for every monadic extension $\Sigma^+$ of $\Sigma$ the class 
$\Cc[\Sigma^+]$ is stable. 

A second important notion is that of \emph{dependence}, defined as follows. 
Let $\phi(\bar x,\bar y)$ be a formula and let~$\struc A$ be a structure. 
A set $A\subseteq \struc A^{|\bar x|}$ is \emph{shattered} by $\phi$ if 
there exists a family $(\bar b_J)_{J\subseteq A}$ of tuples of elements of 
$\struc A$ such that for all $J\subseteq A$ and for all $\bar a\in A$
\[\struc A \models \phi(\bar a, \bar b_J) \quad \Longleftrightarrow \quad 
\bar a\in J.\]

The formula $\phi$ is said to have the \emph{independence property} (IP)
over a class $\Cc$ if it can shatter arbitrarily large sets in structures from $\Cc$. 
Otherwise, it is said to have the \emph{non-independence property (NIP)},
or in a horrible abuse of language, $\phi$ is said to \emph{be NIP over $\Cc$}. 
A class $\Cc$ is \emph{NIP} if every first-order formula is NIP over $\Cc$. 
A class $\Cc$ of $\Sigma$-structures  is \emph{monadically NIP} if 
for every monadic extension $\Sigma^+$ of $\Sigma$ the 
class $\Cc[\Sigma^+]$ is NIP. Note that the concept of dependence
is more general than that of stability, hence, every (monadically) stable class
is (monadically) NIP. 

We call a relation $R$ \emph{definable} on a structure $\struc A$  if
$R = \{\bar a \in \struc A^{|\bar x|} : \struc A\models \phi(\bar a)\}$
for some formula~$\phi(\bar x)$.
The following follows directly from the previous definitions.

\begin{lemma}\label{lem:definable-expansions}
Let $\Cc$ be a monadically stable (monadically NIP) class of 
$\Sigma$-structures, let~$\Sigma^+$ be a monadic extension of 
$\Sigma$ and let $\Dd$ be the hereditary closure of 
any expansion of $\Cc[\Sigma^+]$ by definable relations. Then also $\Dd$
is monadically stable (monadically NIP). 
\end{lemma}

As observed by Baldwin and Shelah in~\cite{baldwin1985second}, 
the expressive power of first-order logic in the colored structures 
$\Cc[\Sigma^+]$ is so strong that in the definitions of monadic stability and 
monadic NIP it suffices to only consider formulas $\phi(x,y)$ with
single free variables instead of tuples $\bar x,\bar y$. 

\begin{lemma}[\cite{baldwin1985second}]\label{lem:mon-stab1}
A class $\Cc$ of $\Sigma$-structures 
is monadically stable (monadically NIP) if and only if for every monadic
extension $\Sigma^+$ of $\Sigma$ every $\Sigma^+$-formula~$\phi(x,y)$ 
is stable (NIP) over~$\Cc[\Sigma^+]$. 
\end{lemma}

A formula $\phi(x,\bar y)$ has \emph{pairing index} $k$ on a class $\Cc$ of
structures if there is $\struc A\in \Cc$ and two sequences 
$(a_{ij})_{1\leq i<j\leq k}$ and $(\bar b_i)_{1\leq i\leq k}$ such that for
all $1\leq i<j\leq k$ and $\ell\in [k]$
\[\struc A \models \phi(a_{ij}, \bar b_{\ell})\quad \Longleftrightarrow\quad \ell \in \{i,j\}.\]

Note that we require that $x$ is a single free variable, while $\bar y$ is allowed
to be a tuple of variables. 
Intuitively, 
from a graph theoretic perspective, a formula has unbounded pairing index if it can encode
arbitrarily large $1$-subdivided cliques, where the principal vertices are represented by tuples and the subdivision vertices are represented by single elements. 

\pairingIndex
\begin{proof}
If a formula $\phi(x,\bar y)$ has unbounded pairing index on $\CC[\Sigma^+]$
then the formula $\psi(\bar x, \bar y) := \exists z. R(z) \land \phi(z,\bar x) \land \phi(z,\bar y)$
can shatter arbitrary large sets over the class of monadic expansions of $\CC[\Sigma^+]$ with one extra unary predicate $R$, making this class monadically independent.
By \Cref{lem:definable-expansions}, $\CC$ is then also monadically independent.

If a class $\CC$ is monadically independent
then by \Cref{lem:mon-stab1}, some formula $\phi(x,y)$ can shatter arbitrary large sets over $\CC[\Sigma^+]$ for some monadic extension $\Sigma^+$.
For every $k$ we can find a set $\{b_1,\dots,b_k\} \subseteq \struc A \in \CC[\Sigma^+]$ shattered by $\phi(x,y)$ via elements $(a_J)_{J\subseteq [k]}$.
The sequences $(a_{\{b_i,b_j\}})_{1\leq i<j\leq k}$ and $(b_i)_{1\leq i\leq k}$
witness that $\phi(x,y)$ has pairing index at least $k$ on $\CC[\Sigma^+]$.
\end{proof}

A similar characterization of monadically NIP classes which does not rely on monadic extensions is given by the notion of \emph{encoding in tuples} in~\cite{braunfeld2021characterizations}.

\paragraph*{Indiscernible sequences.}
Let $\struc A$ be a $\Sigma$-structure and $\phi(\bar x_1,\ldots, \bar x_m)$ a formula. 
We say a sequence $(\bar a_i)_{1\leq i\leq n}$ of tuples from $\struc A$ (where all $\bar x_i$ and $\bar a_j$ have the same length) 
is a \mbox{\emph{$\phi$-indis\-cernible sequence}} of 
length $n$, if for every two sequences of indices
  $i_1 < \dots < i_m$ and
  $j_1 < \dots < j_m$ from $[n]$ we have 
  \[
  \struc A \models 
  \phi(\bar a_{i_1}, \ldots, \bar a_{i_m}) 
  \quad \Longleftrightarrow \quad
  \struc A \models \phi(\bar a_{j_1}, \ldots, \bar a_{j_m}).
  \]
For a set of formulas $\Delta$ we call a sequence
\emph{$\Delta$-indiscernible} if it is $\phi$-indiscernible for 
all $\phi\in \Delta$. 
For any sequence $I=(\bar a_i)_{1\leq i\leq n}$ we define the 
\emph{Ehrenfeucht-Mostowski type (EM-type)} of~$I$ as the
set of all formulas $\phi$ such that $\struc A\models \phi(\bar a_{i_1}, \ldots, \bar a_{i_m})$
for all $i_1<\ldots<i_m$. A sequence $I$ is $\Delta$-indiscernible if
and only if for all formulas $\phi\in \Delta$ either $\phi$ or $\neg\phi$ belongs to 
$\mathrm{EM}(I)$. 

Note that a subsequence $J$ of a $\phi$-indiscernible sequence $I$
is again a $\phi$-indiscernible sequence and that the
$\mathrm{EM}$-type of any subsequence $J$ of a sequence $I$ is a \emph{superset} of the $\mathrm{EM}$-type of $I$. For finite $\Delta$, by (iteratively applying) Ramsey's theorem we can extract
a $\Delta$-indiscernible sequence from any sequence. In general
structures however, in order to extract a large $\Delta$-indiscernible
sequence we must initially start with an enormously large sequence.  To the best of our knowledge the following theorem goes back to Ehrenfeucht and Mostowski~\cite{ehrenfeucht1956models}. 

\begin{theorem}\label{thm:indiscernible_ramsey}
    Let $\Delta$ be a finite set of formulas.
    There exists a function $f$ such that every sequence of elements of length at least $f(m)$ (in a structure with a signature matching $\Delta$)
    contains a $\Delta$-indiscernible subsequence of length $m$.
\end{theorem}

In stable classes we can efficiently find polynomially large indiscernible sequences of elements (see also \cite[Theorem 3.5]{regularity_lemmas}). The theorem is stated for graphs but it easily extend to general structures. 

\begin{theorem}[{\cite[Theorem 2.8]{kreutzer2018polynomial}}]\label{thm:extract_indiscernibles}
  Let $\CC$ be a stable class of graphs and let $\Delta$ be a finite
  set of formulas.  There is a polynomial $p(x)$ such that
  for all $G\in \CC$, every positive integer $m$ and every sequence
  $J$ of vertices of $G$ of length $\ell=p(m)$, there
  exists a subsequence $I$ of length~$m$ which is
  $\Delta$-indiscernible.

  Furthermore, there is an algorithm that given an $n$-vertex graph $G\in \CC$
  and a sequence $(v_i)_{1\leq i\leq \ell}$, computes a
  $\Delta$-indiscernible subsequence of length at
  least $m$. The running time of the algorithm is in
  $O(|\Delta| \cdot k \cdot \ell^{k+1} \cdot n^{q}\cdot a(n)\cdot \lambda(\Delta))$, where $k$
  is the maximal number of free variables, $q$ is the maximal quantifier-rank of
  a formula of $\Delta$, $a(n)$ is the time required to test adjacency between two vertices and
  $\lambda(\Delta)$ is the length of a longest formula in $\Delta$.    
\end{theorem}

By starting with a sequence $(v_i)_{1\leq i\leq \ell'}$ of length $\ell' = p(m)^{k^2+k}$, we know that the number of vertices~$n$ in the host graph is at least $\ell'$.
We may then truncate the sequence to length $\ell=p(m)$ and execute the algorithm of \Cref{thm:extract_indiscernibles}.
The factor $\ell^{k+1} = \ell'^{1/k}$ in the run time can therefore be bounded by $n^{1/k}$,
while still guaranteeing that the starting length $\ell' = p(m)^{k^2+k}$ is only polynomial in $m$.
Looking at the proof in \cite{kreutzer2018polynomial}, we see that
the time needed to evaluate $G \models \phi(\bar v)$ for formulas $\phi \in \Delta$ and tuples $\bar v$
is bounded by $\Oof(n^{q}\cdot a(n)\cdot \lambda(\Delta))$.
Over the course of this paper, we will construct indiscernibles with respect to formulas
that can be evaluated much faster.
To capture this, we only assume a generic bound $f_{\CC\Delta}(n)$ on the evaluation time for formulas in $\Delta$ on $n$-vertex graphs from~$\CC$.
Applying these two modifications to \Cref{thm:extract_indiscernibles}, we immediately get the following statement.

\begin{theorem}\label{thm:poly_seqs}
  Let $\CC$ be a stable class of graphs and let $\Delta$ be a finite set of formulas.
  Assume that we can evaluate, given $\phi \in \Delta$, an $n$-vertex graph 
  $G \in \CC$  and a tuple~$\bar v$ in $G$, whether $G \models \phi(\bar v)$ in time  
  $f_{\CC\Delta}(n)$.

  Then there is an integer $t$ and an algorithm that 
  finds in any sequence of at least $m^t$ vertices in an $n$-vertex graph $G \in\CC$ 
  a $\Delta$-indiscernible subsequence of length $m$.
  The running time of the algorithm is 
  $\Oof(|\Delta| \cdot k \cdot n^{1/k} \cdot f_{\CC\Delta}(n))$, where $k$
  is the maximal number of free variables of formulas in $\Delta$.
\end{theorem}


==> chapters/overview.tex <==
\section{Technical overview}

Our work is organized as follows.
\cref{sec:neighborhoods-ow} introduces useful combinatorial properties of indiscernibles in monadically NIP classes.
We extend those properties in \cref{sec:families-ow}, where we prove our main tool, \Cref{thm:disjoint_families_nip}.
We use this tool in \cref{sec:wideness-ow} to prove flip-flatness.
Due to space constraints, we mostly provide proof sketches, which should convey the key ideas.
%For completeness, a full version for each of these sections is presented in the appendix.
All missing proofs can be found in the full version of the paper~\cite{dreier2022indiscernibles}. 


\input{chapters/overview/ow-neighborhoods.tex}

\input{chapters/overview/ow-families.tex}

\input{chapters/overview/ow-wideness.tex}


==> chapters/overview/ow-families.tex <==
\subsection{Disjoint definable neighborhoods}
\label{sec:families-ow}

In the previous section we have seen that in monadically stable and monadically NIP classes, every element is very homogeneously connected to all but at most one element of an indiscernible sequence.
At a first glance, this exceptional behavior towards one element seems to be erratic and standing in the way of combinatorial and algorithmic applications.
However, it turns out that it can be exploited to obtain additional structural properties.

The key observation is that elements that are ``exceptionally connected'' towards a single element of an indiscernible sequence, inherit some of the good properties of that sequence.
We will give a simple example to demonstrate this idea.
Let $G$ be a graph containing certain red vertices $R$ and blue vertices $B$, such that the edges between $R$ and $B$ describe a matching (see \cref{fig:matching_stars}, left).

\begin{figure}[h]
  \begin{center}
  \includegraphics[scale=0.75]{figures/matching-stars-ipe.pdf}
  \end{center}
  \caption{Examples of one-to-one and many-to-one connections in a graph. On the left: a matching. On the right: a star forest.}
  \label{fig:matching_stars}
\end{figure}

Given a formula $\phi(x_1,\ldots, x_q)$, define 
\[
\hat \phi(x_1,\ldots,x_q)
:= 
\exists b_1,\ldots,b_q \in B. 
\phi(b_1,\ldots,b_q)
\wedge
\bigwedge_{i\in [q]} E(x_i, b_i).
\]

Take a $\hat \phi$-indiscernible sequence $R'$ among $R$.
Obviously, every vertex in the blue neighborhood $B'$ of $R'$ has one exceptional connection towards $R'$, that is, towards its unique matching neighbor in~$R'$.
It is now easy to see that $B'$ is a $\phi$-indiscernible sequence in $G$: for every sequence of red vertices $a_1,\ldots,a_q \in R'$
and their unique blue matching neighbors $b_1,\ldots,b_q \in B'$ we have
$
G\models \hat \phi (a_1,\ldots,a_q )$ if and only if 
$G\models \phi (b_1,\ldots,b_q)$.


This example sketches how first-order definable one-to-one connections
towards elements of an indiscernible sequence preserve indiscernibility.
The more general case however is the many-to-one case,
where we have a set of elements, each of which is exceptionally connected to a single element of an indiscernible sequence $I$, while allowing multiple elements to be exceptionally connected to the same element of $I$
(think, for example, of $R$ and $B$ being the centers and leaves of a star-forest as depicted in \cref{fig:matching_stars}, right).
Our notion of such many-to-one connections will be that of \emph{disjoint $\alpha$-neighborhoods}.
Recall, that for a formula~$\alpha(\bar x,y)$, the \(\alpha\)-neighborhood $N_\alpha(\bar a)$ of a tuple $\bar a$ is defined as the set of all \(b\) satisfying $\alpha(\bar a,b)$.
We say a sequence $J$ of  $|\bar x|$-tuples has \emph{disjoint $\alpha$-neighborhoods} if 
$N_\alpha(\bar a_1)\cap N_\alpha(\bar a_2)=\varnothing$ for all distinct $\bar a_1,\bar a_2\in J$.

As the main technical tool of this paper, we prove for
monadically NIP classes
%controlled connectivity behaviour of single elements not merely to indiscernible sequences but also to sequences of disjoint $\alpha$-neighborhoods.
that every sequence of disjoint $\alpha$-neighborhoods contains a large subsequence that exerts strong control over its neighborhood.
This lifts the strongly regular behaviour of idiscernible sequences to sequences of disjoint $\alpha$-neighborhoods.
The main result of this section, \cref{thm:disjoint_families_nip}, is the backbone of our flip-flatness proof and states the following.
In every large sequence of disjoint $\alpha$-neighborhoods, we will find 
a still-large subsequence such that the $\phi$-connections of every element $a$ towards all $\alpha$-neighborhoods in the subsequence can be described by a bounded set of sample elements in the following sense.
After possibly omitting one exceptional neighborhood at index $\mathrm{ex(a)}$ depending on~$a$,
the \(\phi\)-connections are completely homogeneous (in the stable case) or alternate at most once (in the NIP case).
A related (but orthogonal) result was also proved in \cite[Lemma 64]{twwIVarxiv} using tools from model theory.

\begin{figure}[h]
  \begin{center}
  \includegraphics[scale=1.2]{figures/families-ipe.pdf}
  \end{center}
  \caption{
    A visualization of \cref{thm:disjoint_families_nip}. On the bottom: a sequence $I$ with disjoint $\alpha$-neighborhoods. On the top right: a small set of sample elements $S$.
    The $\phi$-neighborhoods of the elements in $S$ in the $\alpha$-neighborhood of $I$ are colored accordingly. Note that their $\phi$-neighborhoods can overlap.
The $\phi$-neighborhood of $a$ in the $\alpha$-neighborhood of $I$ is equal to the $\phi$-neighborhood of $s_<(a) = s_1$ before the exceptional index $\mathrm{ex}(a)$. After it, it is equal to the $\phi$-neighborhood of $s_>(a) = s_3$. For the $\alpha$-neighborhood of $\bar a_{\mathrm{ex}(a)}$ we make no claims.}
  \label{fig:families}
\end{figure}

\begin{restatable}{theorem}{thmDisjointFamiliesNip}\label{thm:disjoint_families_nip}
For every monadically NIP class of structures $\Cc$, and formulas $\phi(x,y)$ and $\alpha(\bar x,y)$, there exists a function $N:\NN \rightarrow \NN$ and an integer $k$ such that 
for every $m\in \NN$
every structure $\struc A \in \CC$ and every finite sequence of tuples $J\subseteq \struc A^{|\bar x|}$ of length $N(m)$ whose $\alpha$-neighborhoods are disjoint the following holds. 
There exists a subsequence $I =(\bar a_i)_{1\leq i\leq m}\subseteq J$ of length $m$ and a 
set $S \subseteq \struc A$ of at most $k$ sample elements such that for every element $a \in \struc A$ there exists an exceptional index $\mathrm{ex}(a) \in [m]$ and a pair $s_\sless(a),s_\sgreater(a)\in S$ such that 
\begin{alignat*}{2}
    \text{for all }& ~1 \leq i < \mathrm{ex(a)}&&: N_\alpha(\bar a_i) \cap N_\phi(a) = N_\alpha(\bar a_i) \cap N_\phi(s_\sless(a)), \text{ and} \\
    \text{for all }& ~\mathrm{ex(a)} < i \leq m&&: N_\alpha(\bar a_i) \cap N_\phi(a) = N_\alpha(\bar a_i) \cap N_\phi(s_\sgreater(a)).
\end{alignat*}
%
If $a \in N_\alpha(\bar a_i)$ for some $\bar a_i\in I$, then $i = \mathrm{ex}(a)$.

\medskip\noindent
If $\CC$ is monadically stable, then $s_\sless(a) = s_\sgreater(a)$ for every $a\in \struc A$. 
\end{restatable}

A visualization of the NIP case of \cref{thm:disjoint_families_nip} is provided in \cref{fig:families}.
%A full proof of the theorem is given in \Cref{sec:families}.
An important ingredient of the proof is the following Ramsey-type result due to Ding et al.~\cite[Corollary~2.4]{DBLP:journals/jct/DingOOV96}.
We say a bipartite graph with sides $a_1,\ldots, a_\ell$ and $b_1,\ldots, b_\ell$ forms
\begin{itemize}
\item a \emph{matching} of order $\ell$ if $a_i$ and $b_j$ are adjacent if and only if $i=j$ for all $i,j\in [\ell]$, 
\item a \emph{co-matching} of order $\ell$ if $a_i$ and $b_j$ are adjacent if and only if $i\neq j$ for all $i,j\in [\ell]$, 
\item a \emph{ladder} of order $\ell$ if $a_i$ and $b_j$ are adjacent if and only if $i\leq j$ for all $i,j\in [\ell]$. 
\end{itemize}
We call two distinct vertices $u$ and $v$ \emph{twins} in a graph $G$ they have the same neighborhood with regard to the edge relation, i.e. $N_E^G(u) \setminus \{v\} =N_E^G(v) \setminus \{u\}$.

\begin{restatable}[{\cite[Corollary 2.4]{DBLP:journals/jct/DingOOV96}}]{theorem}{thmmatching}\label{thm:matching}
    There exists a function $Q:\NN\rightarrow\NN$ such that for every $\ell\in\NN$ and for every bipartite graph $G = (L,R,E)$ without twins, where $L$ has size at least~$Q(\ell)$, contains a matching, co-matching, or ladder of order $\ell$ as an induced subgraph.
\end{restatable}

Equipped with \cref{cor:iseq_n_mon_stable_multiple_formulas} from the previous subsection and the above \cref{thm:matching}, we will now give a proof sketch of the monadically stable case of \cref{thm:disjoint_families_nip}.

\begin{proof}[Proof sketch of \cref{thm:disjoint_families_nip}
  (monadically stable case)]

We will build the sequence $I$ by inductively extracting indiscernible subsequences $I_i$ of $J$ and growing a set of sample elements $S_i =\{s_1,\ldots,s_i\}$.
During the induction, we maintain the following invariant: 
every two distinct sample elements from~$S_i$ have pairwise different $\phi$-neighborhoods in the $\alpha$-neighborhood of every tuple of~$I_i$.
We start with $I_0 = J$ and $S_0 = \varnothing$ where this trivially holds.
Let us now describe the inductive construction of $I_{i+1}$ and $S_{i+1}$.
We first add a constant symbol for every element in~$S_i$ to the signature of $\struc{A}$. 
This extended signature will allow us to express for all $j\in [i]$ the formula $\psi_j(x, \bar y)$ stating that $x$ has the same $\phi$-neighborhood as $s_j$ in the $\alpha$-neighborhood of $\bar y$, i.e.,
$
  N_\alpha(\bar y) \cap N_\phi(x) = N_\alpha(\bar y) \cap N_\phi(s_j)
$.
We collect all these formulas into the set $\Phi = \{ \psi_j ~:~ j \in [i] \}$ and build $I_{i+1}$ by extracting a $\Delta^\Phi_k$-indiscernible sequence from $I_i$, for the appropriate value of $k$ given by \cref{cor:iseq_n_mon_stable_multiple_formulas}.
Now by \cref{cor:iseq_n_mon_stable_multiple_formulas},
for every element $b \in \struc A$, there exists a $\Phi$-type $\tau(x,\bar{y})$ such that $b$ is $\tau$-connected to all but at most one tuple from~$I_{i+1}$.
Since the \(\Phi\)-types capture information about the connections relative to vertices in \(S_i\),
one of the following two cases applies for every $b \in \struc A$. 
%\todo{Szymon suggests a figure here}
\begin{enumerate}
  \item The $\phi$-neighborhood of $b$ is different to the $\phi$-neighborhood of every element of $S_i$ in the $\alpha$-neighborhood around all but at most one  tuple of~$I_{i+1}$.
  \item For some $j\in [i]$, the $\phi$-neighborhood of $b$ is equal to the $\phi$ neighborhood of $s_j$ in the $\alpha$-neighborhood around all but at most one  tuple of $I_{i+1}$ (whose index will $\mathrm{ex}(b)$).
\end{enumerate}
If the first case applies for some $b \in \struc A$, then we can build $S_{i+1}$ by setting $s_{i+1} := b$, which satisfies our invariant (after we possibly drop one more element from $I_{i+1}$).
If the second case applies for every $b\in \struc A$, every element is represented by $S_i$, and the construction stops with $I := I_{i+1}$ and $S := S_i$.

It now remains to show that the construction stops after less than $k$ steps for some $k$ depending only on $\CC$, $\phi$, and $\alpha$.
To this end, we show that for every $\ell \in \N$, there exists $k\in\N$ with the following property.
If there exists $I_k$ and $S_k$ satisfying the invariant of our construction, then 
we can derive a formula $\psi$ from $\phi$ and $\alpha$ which has pairing index at least~$\ell$ in an expansion of $\struc A$ with a constant number of colors (in the full proof we use 3 colors).
As~$\CC$ is monadically NIP, the pairing index of $\psi$ is bounded, which also yields a bound for $k$.

Assume we are given $I_k$ and $S_k$, such that all the elements from $S_k$ have different $\phi$-neighborhoods, in the $\alpha$-neighborhoods around the tuples of $I_k$.
By choosing \(k\) large enough, repeated application of \cref{thm:matching} and the pigeonhole principle, we find a subset $S' = \{s_1,\ldots,s_{\ell^2}\}$ of $S_k$ and a subsequence $I' = \{\bar a_1, \ldots, \bar a_\ell\}$ of $I_k$ with the following property.
For each $j\in [\ell]$, there exists a subset $N'_j$ of the $\alpha$-neighborhood of $\bar a_j$, such that the \mbox{$\phi$-connections} from $S'$ to the $N'_j$ all form a matching, all form a co-matching, or all form a ladder.
Assume the $\phi$-connections form a matching. Let us now show that the formula
\[
  \psi(x,\bar y) := \exists z \in N_{\phi}(x) \cap N_\alpha(\bar y).\ R(z)
\]
has pairing index at least $\ell$ in the class $\CC$ extended with an additional unary predicate $R$.
The situation is depicted in \cref{fig:families-ow}. 
%
\begin{figure}[h]
    \begin{center}
        \includegraphics[scale=1]{figures/families-ow-ipe.pdf}
    \end{center}
    \caption{Pairing the elements of $I'$.}
    \label{fig:families-ow}
\end{figure}
%
The formulas $\phi$ and $\alpha$ interpret a large 1-subdivided biclique in $\struc A$ as follows. 
The tuples from $I'$ and the elements from $S'$ form the principle vertices.
The subdivision vertices are formed by $\bigcup_{i\in[\ell]}N_i'$. 
Due to the assumed matchings, each subdivision element has exactly one incoming $\phi$-connection from $S'$. 
Due to the tuples in $I'$ having disjoint $\alpha$-neighborhoods, each subdivision element has exactly one incoming $\alpha$-connection from the elements of $I'$. 
Since $I'$ has size~$\ell$ and $S'$ has size $\ell^2$ we can assign 
to every pair $\bar a_i,\bar a_j \in I'$ a unique element $s_{ij} \in S'$.
By marking with the predicate $R$ the two unique subdivision elements from $N_\phi(s_{ij})\cap N_i'$ and $N_\phi(s_{ij})\cap N_j'$, we get that $s_{ij}$ is $\psi$-connected only to $\bar a_i$ and $\bar a_j$ among $I'$.
As desired, $S'$ and $I'$ witness that $\psi$ has pairing index at least $\ell$.

In case the $\phi$-connections form a co-matching or a ladder, we can replace $\phi$ with a derived formula $\phi'$, such that the $\phi'$-connections form a matching in a coloring of $\struc A$, which completes the proof sketch for the size bound of $S$.

Lastly, in order to ensure that $a \in N_\alpha(\bar a_i)$ implies $i = \mathrm{ex}(a)$, we can augment the formula~$\psi_j(x, \bar y)$ in the construction to return false whenever $x$ is contained in $N_\alpha(\bar y)$.
This way, we enforce the single exception given by \cref{cor:iseq_n_mon_stable_multiple_formulas} to be on $a_i$.
\end{proof}

To prove the more general NIP case, we replace \cref{cor:iseq_n_mon_stable_multiple_formulas} with \cref{thm:iseq_n_mon_nip_multiple_formulas}, which introduces the possibility for a vertex $a$ to be sampled by two vertices $s_<(a)$ and $s_>(a)$, alternating around $\mathrm{ex}(a)$.
We also have to slightly adapt the search for the next sample element $s_j$ using an additional indiscernibility argument.


==> chapters/overview/ow-neighborhoods.tex <==
\subsection{Indiscernibles in monadically stable and monadically NIP classes}\label{sec:neighborhoods-ow}

In classical model theory, instead of classes of finite structures, usually infinite structures are studied.
For a single infinite structure $\struc A$, we say 
$\struc{A}$ is (monadically) stable/NIP, if the class $\{\struc{A}\}$ is (monadically) stable/NIP.
In this context, an indiscernible sequence is usually assumed to be of infinite length and 
indiscernible over the set of all first-order formulas.
Using $\Omega$ to denote the set of all first-order formulas, we will denote the latter property as \emph{$\Omega$-indiscernibility}.

It is well-known that indiscernible sequences can be used to characterize stability and NIP for infinite structures.
To characterize NIP, define the \emph{alternation rank} of a formula~$\phi(\bar x,\bar y)$ over a sequence $I$ in a structure $\struc A$ as the maximum~$k$ such that there
exists a (possibly non-contiguous) subsequence $(\bar a_1,\ldots,\bar a_{k+1})$ of $I$ and a tuple $\bar b \in \struc A^{|\bar x|}$ such that for all $i \in [k]$ we have $\struc A \models \phi(\bar b,\bar a_{i}) \iff \struc A \models \neg\phi(\bar b,\bar a_{i+1})$.
A structure $\struc A$ is NIP if and only if every formula has finite alternation rank over every $\Omega$-indiscernible sequence in~$\struc A$ \mbox{\cite[Theorem 12.17]{Poizat}}.
Stable classes can be characterized in a similar way. 
We say the \emph{exception rank} of a formula~$\phi(\bar x,\bar y)$ over a sequence $I$ in a structure $\struc A$ is the maximum~$k$ such that
there exists a tuple $\bar b \in \struc A^{|\bar x|}$ 
such that for $k$ distinct tuples $\bar a_i \in I$ we have $\struc A\models\phi(\bar b, \bar a_i)$
and for $k$ other distinct tuples $\bar a_i \in I$ we have $\struc A\models\neg\phi(\bar b, \bar a_i)$.
A structure $\struc A$ is stable if and only if every formula has finite exception rank over every $\Omega$-indiscernible sequence in $\struc A$ \mbox{\cite[Corollary 12.24]{Poizat}}.

Hence, NIP and stablility can be characterized by the interaction of tuples of elements with indiscernible sequences. 
For \emph{monadically} NIP structures, Blumensath \cite{blumensath2011} shows that the interaction of single elements with indiscernible sequences is even more restricted.

\begin{restatable}[{\cite[{Corollary 4.13}]{blumensath2011}}]{theorem}{thmblumensath}\label{thm:blumensath}
  In every monadically NIP structure $\struc A$, for every formula~$\phi(x,\bar y)$, where $x$ is a single free variable, 
  and $\Omega$-indiscernible sequence $(\bar a_i)_{i \in \N}$ of $|\bar y|$-tuples the following holds:
  for every element $b\in \struc A$
  there exists an exceptional index $\mathrm{ex}(b) \in \N$ and 
  two truth values $t_<(b),t_>(b) \in \{0,1\}$ such that
    \begin{align*}
      &\text{for all } i < \mathrm{ex(b)}: 
      \struc A \models \phi(b,\bar a_i) \hspace{2mm} \iff \hspace{2mm} t_<(b) = 1, \text{ and } \\
      &\text{for all } i > \mathrm{ex(b)}: 
      \struc A \models \phi(b,\bar a_i)\hspace{2mm} \iff \hspace{2mm} t_>(b)=1.
    \end{align*}
\end{restatable}

See \cref{fig:blumensath} for examples. In particular, the alternation rank of the formulas $\phi(x,\bar y)$ with a single free variable $x$ over every $\Omega$-indiscernible sequence in a monadically NIP structure is at most $2$.

\cref{thm:blumensath} will be a crucial tool for proving flip-flatness. 
However, as we strive for algorithmic applications, we have to develop an effective, computable version that is suitable for handling classes of finite structures. Instead of requiring $\Omega$-indiscernibility, we will specifically consider $\Delta$-indiscernible sequences with respect to special sets $\Delta=\Delta^\Phi_k$ that we define soon. These sets $\Delta^\Phi_k$ will strike the right balance of being
on the one hand sufficiently rich to allow us to derive structure from them, but on the other hand
sufficiently simple such that we can efficiently evaluate formulas from $\Delta^\Phi_k$, making our flip-flatness result algorithmic.

\begin{figure}[H]
  \begin{center}
  \includegraphics[scale=1]{figures/blumensath-ipe.pdf}
  \end{center}
  \caption{Two monadically NIP structures. On the left: the infinite half-graph, where \cref{thm:blumensath} applies for the edge relation with $t_<(b) = 0$ and $t_>(b) = 1$.
  On the right: the infinite matching, where
  we have $t_<(b)  = t_>(b) = 0$ but a differing truth value at index $\mathrm{ex}(b) = 3$.
  }
  \label{fig:blumensath}
\end{figure}



Fix a finite set $\Phi(x,\bar{y})$ of formulas of the form $\phi(x,\bar y)$
where $x$ is a single variable.
A \emph{$\Phi$-pattern} is a finite sequence $(\phi_i)_{1\le i\le k'}$,
where each formula $\phi_i(x,\bar y)$
is a boolean combination of formulas $\phi(x,\bar y)\in \Phi(x,\bar y)$.
 Given a $\Phi$-pattern $(\phi_i)_{i\in [k']}$,
the following formula expresses that, 
for a given sequence 
of $k'$ tuples, each of length $|\bar y|$, there is some element that realizes that pattern (see \cref{fig:pattern} for an example):
\[\gamma_{(\phi_1,\ldots,\phi_{k'})}(\bar y_1,\ldots,\bar y_{k'})
=\exists x.\bigwedge_{i\in [k']}\phi_i(x,\bar y_i).\]

For a finite set of formulas $\Phi(x,\bar{y})$ and an integer $k$
we define $\Delta_k^{\Phi}$ to be the set of 
all formulas $\gamma_{(\phi_1,\ldots,\phi_{k'})}$,
where $(\phi_1,\ldots,\phi_{k'})$ is a $\Phi$-pattern of length $k' \leq k$. Note that the set~$\Delta_k^{\Phi}$ is finite, as (up to equivalence) there are only finitely many boolean combinations of formulas in $\Phi$.
We write $\Delta_k^{\phi}$ for $\Delta_k^{\{\phi\}}$.

\begin{figure}[H]
  \begin{center}
  \includegraphics[scale=1]{figures/pattern-ipe.pdf}
  \end{center}
  \caption{Example of an $\{E\}$-pattern: a graph satisfying $G\models \gamma_{(E,E,\neg E,E,\neg E)}(v_1,v_2,v_3,v_4,v_5)$.}
  \label{fig:pattern}
\end{figure}


We can now state a finitary version of \cref{thm:blumensath} as follows.
For the convenient use later~on, we state the result not for single formulas \(\phi\) but for \(\Phi\)-types.
%where we slightly generalize from single formulas $\phi$ to sets of $\Phi$-types for a set of formulas $\Phi$,

\begin{restatable}{theorem}{iseqNMonNipMultipleFormulas}\label{thm:iseq_n_mon_nip_multiple_formulas}
    For every monadically NIP class $\CC$ of structures and finite set of formulas $\Phi(x,\bar y)$ 
    there exist integers $n_0$ and $k$, such that for every 
    $\struc A \in \mathscr{C}$ the following holds. 
    If $I = (\bar a_i)_{1\leq i\leq n}$ is a $\Delta^\Phi_k$-indiscernible sequence of length $n\geq n_0$ in $\struc A$,
    and $b \in \struc A$, 
    then there exists an exceptional index $\mathrm{ex}(b) \in [n]$ and 
    $\Phi$-types $\tau_-(x,\bar y)$ and $\tau_+(x,\bar y)$
    such that
    \begin{alignat*}{2}
        \struc A\models \tau_-(b,\bar a_i) \text{ holds for all }& 1\le i < \mathrm{ex(b)}, \text{ and }
        \\
        \struc A\models \tau_+(b,\bar a_i) \text{ holds for all }& \mathrm{ex}(b)<i\le n.
    \end{alignat*}
\end{restatable}

%We give a proof of \cref{thm:iseq_n_mon_nip_multiple_formulas} in the full version of the paper. 
%\cref{apx:indiscernibles}.
Our proof uses different tools than~\cite{blumensath2011}. It is combinatorial, fully constructive, and gives explicit bounds on $n_0$ and $k$ as well as the required set of formulas $\Delta^\Phi_k$.
One may alternatively finitize \cref{thm:blumensath} via compactness,
but then we do not obtain these crucial properties.

For the more restricted monadically stable classes we can give even stronger guarantees: for every element $b\in\struc A$, the types do not alternate and we have $\tau_- = \tau_+$.

\begin{restatable}{theorem}{iseqNMonStableMultipleFormulas}
  \label{cor:iseq_n_mon_stable_multiple_formulas}
  For every monadically stable class $\CC$ of structures and finite set of formulas~$\Phi(x,\bar y)$
  there exist integers $n_0$ and $k$, such that for every
  $\struc A \in \mathscr{C}$ the following holds.
  If $I = (\bar a_i)_{1\leq i\leq n}$ is a $\Delta^\Phi_k$-indiscernible sequence of length $n\geq n_0$ in $\struc A$,
  and $b \in \struc A$,
  then there exists an exceptional index $\mathrm{ex}(b) \in [n]$ and a $\Phi$-type $\tau$, such that
  \[\struc A\models \tau(b,\bar a_i)
  \qquad\text{for all $i\in [n]$ with
  $i\neq\mathrm{ex}(b)$.}
  \]
\end{restatable}

Building on \cref{thm:iseq_n_mon_nip_multiple_formulas}, we give a full proof of \cref{cor:iseq_n_mon_stable_multiple_formulas}. %in \cref{apx:indiscernibles}. 
In order to give an intuition about the interaction of monadic stability and $\Delta_k^\Phi$-indiscernibility, we sketch a standalone proof here.

\begin{proof}[Proof sketch of \cref{cor:iseq_n_mon_stable_multiple_formulas}]
  

For simplicity, we will focus on the case were $\Phi$ is a singleton set $\{\phi(x, \bar y)\}$.
Let $k$ be the smallest number such that the bound for the pairing index of~$\phi$ and~$\neg\phi$ on $\CC$ is less than $k$.
Such a bound exists since $\CC$ is in particular monadically~NIP.
Assume towards a contradiction that there exists a sufficiently long $\Delta_k^\phi$-indiscernible sequence~$I$ in a structure $\struc A \in \CC$ and an element $b \in \struc A$ that is $\phi$-connected to at least two tuples in $I$ and not $\phi$-connected to at least two other tuples in $I$.
By symmetry, we can assume that $b$ is not $\phi$-connected to the majority of $I$.
We therefore find a length-$k$ subsequence $\bar a_1,\dots,\bar a_k$ of~$I$ and two distinct indices $i_0, j_0 \in [k]$, such that $b$ is $\phi$-connected exactly to the $i_0$th and $j_0$th element of \(\bar a_1,\dots,\bar a_k\). 
We say that the $i_0$th and $j_0$th element are \emph{$\phi$-paired} by \(b\).
Our goal is to derive a contradiction by finding also for every other pair \(i,j\) of indices an element that \(\phi\)-pairs them,
%additional elements which $\phi$-pair every other pair in $J$,
witnessing that $\phi$ has pairing index at least $k$ in $\CC$.


In stable classes, every sufficiently long $\Delta_k^\phi$-indiscernible sequence $I$ is also \emph{totally $\Delta_k^\phi$-indiscernible}: This means that every permutation $I'$ of $I$ is again $\Delta_k^\phi$-indiscernible, with the formulas from $\Delta_k^\phi$ taking the same truth values on $I'$ as on \(I\).
Intuitively speaking, if permuting two elements in an indiscernible sequence would change the truth value of a formula, then this formula orders these two elements and by indiscernibility also orders a large part of the sequence, contradicting stability.
A proof of the statement for $\Omega$-indiscernibles can be found in \cite[Lemma 9.1.1]{tent2012course}. 

%To pair index \(i\) and \(j\), let
%$J'$ be the permutation of $J$ where the $i_0$th and $i$th, and the $j_0$th and $j$th element of $J$ are swapped.

The formula \(\gamma(\bar y_1, \ldots, \bar y_k)
    :=
    \text{ ``$\bar y_{i_0}$ and $\bar y_{j_0}$ are \(\phi\)-paired by some element''}\) is contained in $\Delta_k^\phi$ and holds on \(\bar a_1,\dots,\bar a_k\), as witnessed by \(b\).
By total indiscernibility, we may permute \(\bar a_1,\dots,\bar a_k\) and the formula still holds.
By swapping \(a_{i_0}\) with \(a_i\) and \(a_{j_0}\) with \(a_j\),
we obtain for arbitrary \(i,j\) that
``$\bar a_{i}$ and $\bar a_{j}$ are \(\phi\)-paired by some element''.
This witnesses that \(\phi\) has pairing index at least~\(k\), a contradiction.
\end{proof}

%``there exists an element which $\phi$-pairs $\bar y_i$ and $\bar y_j$ of $(\bar y_1, \ldots, \bar y_k)$''.


%To this end we will exploit the stability of $\CC$ using the following claim.
%
%\begin{claim}\label{claim:totally_indiscernible}
%  In stable classes we have that every sufficiently long $\Delta_k^\phi$-indiscernible sequence $I$ is also \emph{totally} $\Delta_k^\phi$-indiscernible: every permutation $I'$ of $I$ is again $\Delta_k^\phi$-indiscernible, with the formulas from $\Delta_k^\phi$ taking the same truth values on $I'$, i.e. $\mathrm{EM}(I) \cap \Delta_k^\phi = \mathrm{EM}(I') \cap \Delta_k^\phi$.
%\end{claim}
%
%Intuitively, if permuting two elements $a_1$ and $a_2$ in an indiscernible sequence changes the truth value of a formula $\psi$, then $\psi$ orders $a_1$ and $a_2$ and by indiscernibility also orders a large part of the sequence, contradicting stability.
%A proof of the claim for $\Omega$-indiscernibles can be found in \cite[Lemma 9.1.1]{tent2012course}.
%
%Using \cref{claim:totally_indiscernible}, we will now argue that for every distinct $i,j \in [k]$, there exists an element which $\phi$-pairs the $i$th and $j$th element of $J$.
%Let $I_{ij}$ be the permutation of $I$ where the $i_0$th and $i$th, and the $j_0$th and $j$th element of $J$ are swapped.
%By construction, $I_{ij}$ contains a subsequence $J_{ij}$ (which is a permutation of $J$) of length-$k$, where $b$ pairs the $i$th and $j$th element.
%Note that the formula
%\[
%  \gamma_{ij}(\bar y_1, \ldots, \bar y_k)
%  :=
%  \text{ ``there exists an element which $\phi$-pairs $\bar y_i$ and $\bar y_j$ of $(\bar y_1, \ldots, \bar y_k)$''}
%\]
%is contained in $\Delta_k^\phi$.
%As witnessed by $b$ and $J_{ij}$ we have $\gamma_{ij} \in \mathrm{EM}(I_{ij})$.
%Now by \cref{claim:totally_indiscernible} we also have $\gamma_{ij} \in \mathrm{EM}(I_{ij})$ meaning that for every $k$ element subsequence of $I$, in particular for $J$, there exists an element which $\phi$-pairs the $i$th and $j$th element.
%\end{proof}

For the more general monadically NIP case, we cannot rely on total indiscernibility. 
Instead, we bound the alternation rank by pairing tuples located around alternation points, leading to a similar but more involved reasoning.

\begin{figure}[H]
  \begin{center}
  \includegraphics[scale=0.70]{figures/indiscernible-neighbourhoods-ipe.pdf}
  \end{center}
  \caption{All types of neighborhoods a vertex (top) can have in indiscernible
    sequences (bottom) in different graph classes.}
  \label{fig:sparse_inclusion_diagramm0}
\end{figure}

We conclude this section by mentioning that a behavior similar to \cref{cor:iseq_n_mon_stable_multiple_formulas} was already observed in \cite{kreutzer2018polynomial} for the edge relation in nowhere dense classes.
Considering only the edge relation, we depict the different possible behavior of vertices towards indiscernible sequences in different classes of graphs in \cref{fig:sparse_inclusion_diagramm0}.
In monadically NIP (or stable) classes, the same six (or four) patterns apply for connections with respect to any formula \(\phi(x,y)\).





==> chapters/overview/ow-wideness.tex <==
\subsection{Flatness in monadically stable classes of graphs}\label{sec:wideness-ow}

In this section we use \cref{thm:disjoint_families_nip} to characterize monadically stable graph classes in terms of flip-flatness. 
We start with the forward direction, restated for convenience.

\thmfuqwforward*

\begin{proof}[Partial proof]
    Let $\CC$ be a monadically stable class of graphs and $r\in \NN$. 
    We want to show that in every graph $G\in \CC$, in every set $A \subseteq V(G)$ of size $N_{r}(m)$ we find a subset $B\subseteq A$ of size at least $m$ and a set $F$ of at most $s_{r}$ flips such that $B$ is distance-$r$ independent in $G\oplus F$.
    We will first inductively describe how to obtain the set of vertices $B$ and the set of flips $F$ and bound the runtime and values for $N_r$ and $s_r$ later.
    In the base case we have $r=0$. We can pick $B := A$ and $F := \varnothing$ and there is nothing to show.

    In the inductive case we assume the result is proved for $r$ and extend it to $r+1$.
    Let $r = 2i + p$ for some $i\in \NN$ and parity $p\in \{0,1\}$.
    Apply the induction hypothesis to obtain $s_r$ flips $F_r$ and a set $A_r$ that  is distance-$r$ independent in $G_r := G \oplus F_r$.
    Note that for every fixed number $t$ of flips, since flips are definable by coloring and a quantifier-free formula, the class $\Cc_t$ of all graphs obtainable from graphs of $\Cc$ by at most $t$ flips is monadically stable by~\cref{lem:definable-expansions}. Hence, $G_r$ comes from the monadically stable class~$\CC_{s_r}$.
    Our goal is to find a set of flips $F'_{r+1}$ (of fixed finite size which will determine the number $s_{r+1}$) together with a set $A_{r+1} \subseteq A_r$, that is distance-$(r+1)$ independent in $G_{r+1} := G_r \oplus F'_{r+1}$.
    Then $G_r = G \oplus F_{r+1}$ with $F_{r+1} = F_r \cup F'_{r+1}$.

    Since the elements in $A_r$ have pairwise disjoint distance-$i$ neighborhoods, we can apply \cref{thm:disjoint_families_nip} to $A_r$ with $\phi(x,y)=E(x,y)$ and $\alpha(x,y) = \mathrm{dist}_{\leq i}(x,y)$.
    Since we are in the monadically stable case, this yields a subset $A_{r+1} \subseteq A_r$ and a small set of sample vertices $S$ such that for every vertex $a\in V(G)$ there exists $s(a) \in S$ and $\mathrm{ex}(a)\in A_{r+1}$ such that $a$ has the same edge-neighborhood as $s(a)$ in the distance-$i$ neighborhoods of all elements from $A_{r+1}\setminus \{\mathrm{ex}(a)\}$.
    We now do a case distinction depending on whether $r$ is even or odd.

    \paragraph*{The odd case: $\boldsymbol{r=2i + 1}$.}
    For every $s \in S$ let $C_s$ be the set containing every vertex $a$ for which we have $s(a) = s$ and that is at distance at least $i+1$ from every vertex in $A_{r+1}$.
    Let~$D_s$ be the set containing every edge-neighbor of $s$ that is at distance exactly $i$ from one of the vertices in $A_{r+1}$.
    We now build the set of flips $F'_{r+1}$ by adding for every sample vertex $s \in S$ the flip $(C_s,D_s)$.

    Let us now argue that $A_{r+1}$ is distance-$(r+1)$ independent in $G_{r+1}:= G_r$.
    We only flip edges in $G_r$ between pairs of vertices $a,b$
    such that $a$ has distance (in $G_r$) at least $i+1$ and $b$ has distance exactly $i$ to $A_{r+1}$.
    It follows that $A_{r+1}$ remains distance-$(2i + 1)$ independent in $G_{r+1}$.
    Assume towards a contradiction that there exists a path $P = (a,a_1,\ldots,a_i,u,b_i,\ldots,b_1,b)$ of length $r+1=2i+2$ between two vertices $a,b \in A_{r+1}$ in~$G_{r+1}$.
    The distance between~$a$ and~$a_i$ (resp. $b$ and $b_i$) is not affected by the flips. Only the connection between $a_i$ (resp. $b_i$) and $u$ can possibly be impacted.
    Additionally, note that $u\in C_{s(u)}$.

    Since $a$ and $b$ are distinct we have that either $\mathrm{ex}(u) \neq a$ or $\mathrm{ex}(u) \neq b$. By symmetry we can assume the former case.
    As $a_i$ is in the distance-$i$ neighborhood of $a$, we have $G_r\models E(u,a_i) \iff  G_r \models E(s(u),a_i)$.
    %
    Observe that if $E(s(u),a_i)$ holds in $G_r$, then $a_i \in D_{s(u)}$ and therefore the edge $(u,a_i)$ was removed by the flips and is not in $G_{r+1}$.
    Similarly, if $E(s(u),a_i)$ does not hold in $G_r$, then $a_i \not\in D_{s(u)}$
    and the edge $(u,a_i)$ was not introduced by any flip.
    %
    We can conclude that $P$ is not a path in~$G_{r+1}$, and that
    $A_{r+1}$ is distance-$(r+1)$ independent in $G_{r+1}$.

    \paragraph*{The even case and runtime analysis.}
    The even distance creates a symmetry that requires additional care to handle, but otherwise proceeds similarly to the odd case.
    %Due to space constraints, this case was moved to \cref{sec:wideness}.
    The arguments concerning size bounds and runtimes can be found there as well.
    The runtime bound crucially uses the fact that we take \(\Delta^\Phi_k\)-indiscernible sequences only with respect to formulas \(\Phi\) that can be evaluated in polynomial time.
\end{proof}

We have shown that for graph classes, monadic stability implies flip-flatness. We now show that the reverse holds as well.
We will use the following statement, which is an immediate consequence of Gaifman's locality theorem~\cite{gaifman82}.
For an introduction of the locality theorem see for example~\cite[Section 4.1]{grohe2008logic}.

\begin{restatable}[of {\cite[Main Theorem]{gaifman82}}]{corollary}{gaifmancoloring}\label{lem:gaifman-coloring}
%\begin{corollary}[of \cite{gaifman82}]\label{lem:gaifman-coloring}
  Let $\phi(x,y)$ be a formula. Then there are numbers $r,t\in \NN$, where $r$ depends only on the quantifier-rank of $\phi$ and $t$ depends only on the signature and quantifier-rank of $\phi$,
  such that every (colored) graph $G$ can be vertex-colored using $t$ colors
  in such a way that for any two vertices $u,v\in V(G)$ with distance greater than $r$ in $G$,
  $G\models\phi(u,v)$ depends only on the colors of $u$ and $v$.
  We call $r$ the \emph{Gaifman radius} of $\phi$.
%\end{corollary}
\end{restatable}

\begin{restatable}{lemma}{fuqwbackward}\label{lem:fuqw_backward}
%\begin{lemma}\label{lem:fuqw_backward}
    Every flip-flat class of graphs is monadically stable.
%\end{lemma}
\end{restatable}

\begin{proof}[Proof sketch of \cref{lem:fuqw_backward}]
    Assume towards a contradiction that there exists a class $\CC$ that is not monadically stable but flip-flat.
    Then there exists a formula $\sigma(x,y)$ and a graph $G\in\CC$, such that $\sigma$ defines an order on a large vertex set $A$ in a coloring $G^+$.
    Let~$r$ be the Gaifman radius of $\sigma$.
    By flip-flatness there exists a (still large) subset $B$ of $A$ and a bounded size set of flips $F$, such that $B$ is distance-$r$ independent in $H := G^+ \oplus F$.
    Let~$H^+$ be the graph where we have marked the flips $F$ with colors in $H$. 
    We can rewrite $\sigma$ to a formula $\sigma'$ of the same quantifier rank such that for all $u,v\in V(G)$ we have
    $H^+ \models \sigma'(u,v)$ if and only if $G^+ \models \sigma(u,v)$.
    In particular, $\sigma'$ orders $B$ in $H^+$.
    By \cref{lem:gaifman-coloring} and the pidgeonhole principle, there must be two distinct vertices $u,v \in B$ such that $H^+ \models \sigma'(u,v)$ if and only if $H^+ \models \sigma'(v,u)$. However as $\sigma'$ orders $B$, we also have $H^+ \models \sigma'(u,v)$ if and only if $H^+ \not\models \sigma'(v,u)$; a contradiction.
\end{proof}

From \cref{thm:fuqw_forward} and \cref{lem:fuqw_backward} we conclude the following.

\thmfuqw*
%\begin{restatable*}{theorem}{fuqw}\label{thm:fuqw}
%%\begin{theorem}\label{thm:fuqw}
%    A class of graphs is monadically stable if and only if it is flip-flat.
%%\end{theorem}
%\end{restatable*}

